Non-Visible Light Data Synthesis and Application: A Case Study for Synthetic Aperture Radar Imagery

We explore the "hidden" ability of large-scale pre-trained image generation models, such as Stable Diffusion and Imagen, in non-visible light domains, taking Synthetic Aperture Radar (SAR) data for a case study. Due to the inherent challenges in capturing satellite data, acquiring ample SAR training samples is infeasible. For instance, for a particular category of ship in the open sea, we can collect only few-shot SAR images which are too limited to derive effective ship recognition models. If large-scale models pre-trained with regular images can be adapted to generating novel SAR images, the problem is solved. In preliminary study, we found that fine-tuning these models with few-shot SAR images is not working, as the models can not capture the two primary differences between SAR and regular images: structure and modality. To address this, we propose a 2-stage low-rank adaptation method, and we call it 2LoRA. In the first stage, the model is adapted using aerial-view regular image data (whose structure matches SAR), followed by the second stage where the base model from the first stage is further adapted using SAR modality data. Particularly in the second stage, we introduce a novel prototype LoRA (pLoRA), as an improved version of 2LoRA, to resolve the class imbalance problem in SAR datasets. For evaluation, we employ the resulting generation model to synthesize additional SAR data. This augmentation, when integrated into the training process of SAR classification as well as segmentation models, yields notably improved performance for minor classes

==> fig/appfig_prompt.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/fig_chat_v2.00.pdf}
    \caption{\textbf{Prompt construction.} 
    We use GPT-4~\citep{OpenAI2023GPT4TR} to construct high-quality prompts for ORS data. The robot emoji indicates the GPT-4-0314 LLM engine.\qianru{if no space in the main paper, this can be moved to Appendix. Please refer to it if it is moved.} \zc{I will replace it with a pLoRA illustration, I can make it by 14 Nov.}}
    \label{fig:prompt}
\end{figure*}

==> tab/apptab_16attrilora.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{$K$-means clustering with $k=16$.}}
\label{tab:16attrilora}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrrrrrrrrrrrrr@{}}
\toprule[1.3pt]
Category & $C_1$ & $C_2$ & $C_3$ & $C_4$ & $C_5$ & $C_6$ & $C_7$ & $C_8$ & $C_9$ & $C_{10}$ & $C_{11}$ & $C_{12}$ & $C_{13}$ & $C_{14}$ & $C_{15}$ & $C_{16}$ \\ \midrule \midrule
Cargo & 162 & 415 & 52 & 583 & 264 & 307 & 6 & 196 & 34 & 47 & 169 & 445 & 2 & 224 & 475 & 1 \\
Other & 7 & 17 & 3 & 82 & 20 & 29 & 0 & 1 & 1 & 0 & 10 & 75 & 0 & 13 & 14 & 0 \\
Fishing & 18 & 45 & 23 & 64 & 30 & 70 & 19 & 95 & 122 & 39 & 74 & 44 & 0 & 209 & 62 & 2 \\
Tanker & 15 & 89 & 11 & 246 & 86 & 68 & 14 & 130 & 396 & 44 & 68 & 139 & 13 & 423 & 174 & 7 \\
Dredger & 26 & 24 & 0 & 171 & 23 & 27 & 0 & 3 & 1 & 3 & 2 & 44 & 0 & 9 & 22 & 0 \\ \midrule
All & 228 & 590 & 89 & 1,146 & 423 & 501 & 39 & 425 & 554 & 133 & 323 & 747 & 15 & 878 & 747 & 10 \\ \bottomrule[1.3pt]
\end{tabular}
}
\end{table}


==> tab/apptab_2attrilora.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{$K$-means clustering with $k=2$.}}
\label{tab:2attrilora}
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{}}
\toprule
 & Cargo & Other & Fishing & Tanker & Dredger \\ \midrule
Original & 3,890 & 1,710 & 814 & 315 & 242 \\
Attribute 1 & 2,749 & 972 & 597 & 206 & 122 \\
Attribute 2 & 1,141 & 738 & 217 & 109 & 120 \\ \midrule
Ratio & 0.71:0.29 & 0.56:0.44 & 0.73:0.27 & 0.35:0.65 & 0.5:0.5 \\ \bottomrule
\end{tabular}
}
\end{table}

==> tab/apptab_fusar.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule[1.3pt]
Category & Cargo & DiveVessel$^\dagger$ & Dredger & Fishing & HighSpeedCraft$^\dagger$ & LawEnforce$^\dagger$ & Other$^\ast$ & Passenger$^\dagger$ \\ \midrule
Test Sample & 325 & 1 & 14 & 120 & 3 & 3 & 412 & 6 \\ \bottomrule[1.3pt] \addlinespace[0.05em] \cmidrule[1.3pt](r){1-8}
Category & PortTender$^\dagger$$^\ast$ & Reserved$^\dagger$$^\ast$ & SAR$^\dagger$ & Tanker & Tug$^\dagger$ & Unspecified$^\ast$ & WingInGrnd$^\dagger$$^\ast$ &  \\ \cmidrule(r){1-8}
Test Sample & 1 & 9 & 2 & 34 & 9 & 14 & 2 &  \\ \cmidrule[1.3pt](r){1-8}
\end{tabular}
}
\caption{\textbf{Sample numbers of FUSAR dataset.} The FUSAR dataset faces problems of insufficient test samples and vaguely defined classes. Categories marked by ``$\dagger$" means it is deprecated due to insufficient test samples, and ``$\ast$" means being vaguely defined. Results are shown in classification F1-Score, and ``IM21K" indicates pre-trained ResNet50 on the IM21K dataset.}
\label{tab:fusar}
\end{table*}

==> tab/tab_fusarmap.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule[1.3pt]
\multirow{2}{*}{Category} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Augmented} \\ \cmidrule(l){2-5} 
 & Samples & Pixel (\%) & Aug Samples & Pixel (\%) \\ \midrule \addlinespace[0.05em] \midrule 
Water & 3,136 & 18.06 & - & 14.31 \\
Trees & 5,744 & 17.91 & - & 15.19 \\
Building & 5,220 & 11.95 & \textbf{+2,106} & \textbf{15.34} \\
Road & 5,210 & 5.66 & \textbf{+2,329} & \textbf{14.97} \\
Others & 6,093 & 46.39 & - & 40.19 \\ \bottomrule[1.3pt]
\end{tabular}
}
\caption{\textbf{FUSAR-Map dataset statistics}. We resample minor classes ``Road" and ``Building" to achieve approximately 15\% pixel proportion.}
\label{tab:fusarmap}
\end{table}


==> tab/tab_fusrs.tex <==
\begin{table}[t]
\centering
\resizebox{0.98\linewidth}{!}{%
\begin{tabular}{@{}clrrrrr@{}}
\toprule[1.3pt]
Index & Name & Train & Deci & Val & Test & Total \\ \midrule \addlinespace[0.05em] \midrule 
0 & Cargo & 3,890 & 389 & 484 & 772 & 5,146 \\
1 & Other & 1,710 & 171 & 213 & 216 & 2,139 \\
2 & Fishing & 814 & 81 & 102 & 161 & 1,077 \\
3 & Tanker & 315 & 32 & 40 & 59 & 414 \\
4 & Dredger & 242 & 24 & 30 & 52 & 324 \\ \midrule
 & Total & 6,971 & 696 & 869 & 1,260 & 9,100 \\ \bottomrule[1.3pt]
\end{tabular}
}
\caption{\textbf{FU-SRS dataset statistics.} The ``Deci" set is a 1/10 subset of the training set. \zc{Will merge Tables 1 and 2 into a single histogram plot, using two histogram figures to show statistics.}}
\label{tab:fusrs}
\end{table}
